Complexity-calibrated Benchmarks for Machine Learning Reveal When Next-Generation Reservoir Computer Predictions Succeed and Mislead

Recurrent neural networks are used to forecast time series in finance, climate, language, and from many other domains. Reservoir computers are a particularly easily trainable form of recurrent neural network. Recently, a "next-generation" reservoir computer was introduced in which the memory trace involves only a finite number of previous symbols. We explore the inherent limitations of finite-past memory traces in this intriguing proposal. A lower bound from Fano's inequality shows that, on highly non-Markovian processes generated by large probabilistic state machines, next-generation reservoir computers with reasonably long memory traces have an error probability that is at least ~ 60% higher than the minimal attainable error probability in predicting the next observation. More generally, it appears that popular recurrent neural networks fall far short of optimally predicting such complex processes. These results highlight the need for a new generation of optimized recurrent neural network architectures. Alongside this finding, we present concentration-of-measure results for randomly-generated but complex processes. One conclusion is that large probabilistic state machines -- specifically, large $\epsilon$-machines -- are key to generating challenging and structurally-unbiased stimuli for ground-truthing recurrent neural network architectures.

==> cmechabbrev.tex <==
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}  {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\SampleSpace} { \AllPasts }
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\MeasSymbols}[2]{ \MeasSymbol_{#1:#2} }
\newcommand{\meassymbols}[2] { \meassymbol_{#1:#2} }
\newcommand{\BiInfinity}    { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}    { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past} { \smash{\overleftarrow {\MeasSymbol}} }
%\newcommand{\Past} { \MeasSymbols{}{0} }
\newcommand{\past} { {\smash{\overleftarrow {\meassymbol}}} }
%\newcommand{\past} { \meassymbols{}{0} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}   { \smash{\overrightarrow{\MeasSymbol}} }
%\newcommand{\Future} { \MeasSymbols{0}{} }
\newcommand{\future}   { \smash{\overrightarrow{\meassymbol}} }
%\newcommand{\future} { \meassymbols{0}{} }
\newcommand{\futureprime}   { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}   { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}  { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL} { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL} { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}    { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}  { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}    { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }
\newcommand{\rep}    { r }
\newcommand{\Rep}    { \mathcal{R} }
\newcommand{\repa}    { \widehat{r} }
\newcommand{\Repa}    { \widehat{\mathcal{R}} }
\newcommand{\repb}    { \widetilde{r} }
\newcommand{\Repb}    { \widetilde{\mathcal{R}} }


\newcommand{\Present} {\MeasSymbol_0}

% Causal states and epsilon-machines
\newcommand{\CausalState}   { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}   { \sigma }
\newcommand{\CausalStateSet}    { \bm{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}   { \AlternateState^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}   { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \bm{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \bm{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}  { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}  { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}     { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}       {C_\mu}
\newcommand{\hmu}       {h_\mu}
\newcommand{\EE}        {{\bf E}}
\newcommand{\TI}        {{\bf T}}
\newcommand{\SI}        {{\bf S}}
\newcommand{\SE}        { H_{\mathrm{sync}} }
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}        {\chi}

% Causal Irreversibility
\newcommand{\CI}        {\Xi}
\newcommand{\ReverseMap}    {r}
\newcommand{\ForwardMap}    {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\mathbf{\EstCausalState}}
\newcommand{\EstCausalFunc} {\widehat{\epsilon}}
\newcommand{\EstCmu}        {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}    { \mathcal{A}}
\newcommand{\insymbol}      { a}
\newcommand{\OutAlphabet}   { \mathcal{B}}
\newcommand{\outsymbol}     { b}
\newcommand{\InputSimple}   { X}
\newcommand{\inputsimple}   { x}
\newcommand{\BottleneckVar} {\tilde{\InputSimple}}
\newcommand{\bottleneckvar} {\tilde{\inputsimple}}
\newcommand{\InputSpace}    { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}   { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}   { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}    { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}  { Y}
\newcommand{\outputsimple}  { y}
\newcommand{\OutputSpace}   { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}    { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}    { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}  { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}  { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne} { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone} { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}    {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}    {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}   {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}    {{\InputPast}^{L}}
\newcommand{\inputpastL}    {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}  {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}  {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts} { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \mathbf{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}  { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}  { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}   { \mathcal{F}}
\newcommand{\feedbackcausalstate}   { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}      { \mathcal{J}}
\newcommand{\JointCausalStateSet}   { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}   { {\Omega}}
\newcommand{\naturestate}   { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}   { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}   {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}           { {\widehat{\Prob}_N}}
\newcommand{\STRegion}          { {\mathrm K}}
\newcommand{\STRegionVariable}      { K}
\newcommand{\stregionvariable}      { k}
\newcommand{\GlobalPast}        { \overleftarrow{G}}
\newcommand{\globalpast}        { \overleftarrow{g}}
\newcommand{\GlobalFuture}      { \overrightarrow{G}}
\newcommand{\globalfuture}      { \overrightarrow{g}}
\newcommand{\GlobalState}       { \mathcal{G}}
\newcommand{\globalstate}       { \gamma}
\newcommand{\GlobalStateSet}        { {\mathbf \GlobalState}}
\newcommand{\LocalPast}         { \overleftarrow{L}}
\newcommand{\localpast}         { \overleftarrow{l}}
\newcommand{\AllLocalPasts}     { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}       { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}       { \overrightarrow{L}}
\newcommand{\localfuture}       { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}     { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}        { \mathcal{L}}
\newcommand{\localstate}        { \lambda}
\newcommand{\LocalStateSet}     { {\mathbf \LocalState}}
\newcommand{\PatchPast}         { \overleftarrow{P}}
\newcommand{\patchpast}         { \overleftarrow{p}}
\newcommand{\PatchPastRegion}       { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}       { \overrightarrow{P}}
\newcommand{\patchfuture}       { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}     { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}        { \mathcal{P}}
\newcommand{\patchstate}        { \pi}
\newcommand{\PatchStateSet}     { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}    {\vec{\LocalState}}
\newcommand{\localstatesinpatch}    {\vec{\localstate}}
\newcommand{\PointInstantX}     { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}         { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}    {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]    { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]    { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]      { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]      { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}  { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess} { {\Process}^{\forward} }
\newcommand{\PastProcess}   { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}  { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}     { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}     { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}  { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}    { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}      { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}     { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps} { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}        {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}    { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}    { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SGBE}[2][0]{
  \ensuremath{H[\CausalState_{#2} | \MeasSymbols{#1}{#2}]}
}

\newcommand{\GI}{\varphi}
\newcommand{\OI}{\zeta}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{k_{\PC}}
\newcommand{\GOrder}{k_{\GI}}
\newcommand{\OOrder}{k_{\OI}}
\newcommand{\MOrder}{R}
\newcommand{\SOrder}{k_{\SI}}
\newcommand{\Lsync} {\mathcal{L}_{\mathrm{sync}}}

%% stuff for the anatomy paper

\newcommand{\rhomu}{\rho_\mu}
\newcommand{\rmu}{r_\mu}
\newcommand{\bmu}{b_\mu}
\newcommand{\qmu}{q_\mu}
\newcommand{\wmu}{w_\mu}
\newcommand{\imu}{i_\mu}
\newcommand{\sigmamu}{\sigma_\mu}
\newcommand{\EER}{\EE_R}
\newcommand{\EEB}{\EE_B}
\newcommand{\EEQ}{\EE_Q}
\newcommand{\EEW}{\EE_W}
\newcommand{\I}{\mathbf{I}}

%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}

%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi




